Reinforcing Competitive Multi-Agents for Playing 'So Long Sucker'

This paper investigates the strategy game So Long Sucker (SLS) as a novel benchmark for multi-agent reinforcement learning (MARL). Unlike traditional board or video game testbeds, SLS is distinguished by its coalition formation, strategic deception, and dynamic elimination rules, making it a uniquely challenging environment for autonomous agents. We introduce the first publicly available computational framework for SLS, complete with a graphical user interface and benchmarking support for reinforcement learning algorithms. Using classical deep reinforcement learning methods (e.g., DQN, DDQN, and Dueling DQN), we train self-playing agents to learn the rules and basic strategies of SLS. Experimental results demonstrate that, although these agents achieve roughly half of the maximum attainable reward and consistently outperform random baselines, they require long training horizons (~2000 games) and still commit occasional illegal moves, highlighting both the promise and limitations of classical reinforcement learning. Our findings establish SLS as a negotiation-aware benchmark for MARL, opening avenues for future research that integrates game-theoretic reasoning, coalition-aware strategies, and advanced reinforcement learning architectures to better capture the social and adversarial dynamics of complex multi-agent games.

==> 3proposed.tex <==



\section{Proposed Methodology}
\label{3sec:method}

\subsection{Preliminaries of Reinforcement Learning}
\label{sec:preliminaries}

Reinforcement Learning (RL) is a machine learning paradigm where an agent interacts with an environment to maximize cumulative reward. Formally, the problem is modeled as a Markov Decision Process (MDP) defined by:

\begin{itemize}
    \item \textbf{State space} $\mathcal{S}$: the set of all possible environment states.
    \item \textbf{Action space} $\mathcal{A}$: the set of all actions available to the agent.
    \item \textbf{Transition function} $P(s'|s,a)$: the probability of moving from state $s$ to $s'$ given action $a$.
    \item \textbf{Reward function} $R(s,a,s')$: a scalar signal returned for transition $(s,a,s')$.
    \item \textbf{Policy} $\pi(a|s)$: the agent’s strategy for selecting an action in state $s$.
\end{itemize}

\noindent
The goal is to find an optimal policy $\pi^*$ that maximizes the expected discounted return:
\begin{equation}
    G_t = \sum_{k=0}^{\infty} \gamma^k R_{t+k+1}, 
\end{equation}
where, $\gamma \in [0,1)$ balances short/ long-term rewards. Classical algorithms include value-based methods (DQN, DDQN, Dueling DQN), policy-based methods, and actor–critic hybrids.



\subsection{State, Action, and Reward Representation}
We formulate SLS as an RL environment with structured state, action, and reward definitions.

\paragraph{State ($s_t$).}  
The state at time $t$ encapsulates: (i) the board configuration, (ii) chips held by each player, (iii) eliminated (dead) chips, (iv) the current player, (v) the game phase, and (vi) the step count:
\begin{equation}
    s_t = \{\text{Board}, \text{Player Chips}, \text{Dead Chips}, 
    \text{Current Player}, \text{Game Phase}, \text{Steps}\}.
\end{equation}

The observation space size is:
\begin{equation}
\text{total\_obs\_size} = \text{num\_rows} \times \text{num\_players} \times \text{max\_pile\_size} +
\text{num\_players}^2 + 2 \times \text{num\_players} + 4 + 1,
\end{equation}
covering board configuration, chip ownership, elimination flags, current player encoding, game-phase encoding, and step tracking.

\paragraph{Action ($a_t$).}  
The discrete action space is
\begin{equation}
    \mathcal{A} = \{0,1,2,3,4,5,6,7,8,9\},
\end{equation}
with two groups: (i) $\{0,\dots,5\}$ for selecting piles (\texttt{choose\_pile}), and (ii) $\{6,\dots,9\}$ for selecting a player (\texttt{choose\_chip}, \texttt{choose\_next\_player}, \texttt{eliminate\_chip}).  

\paragraph{Reward ($r_t$).}  
Rewards are designed to encourage legal and efficient play:
\begin{itemize}
    \item Illegal moves incur $-5$ penalty.  
    \item Legal moves start with reward $+5$, dynamically adjusted by the number of steps taken:
\end{itemize}
\begin{equation}
    r_t = \min\left(5, \frac{5}{\alpha \cdot \text{steps}}\right), 
\end{equation}
where
\begin{equation}
    \alpha = \frac{15}{\text{chips} \times \beta}, \quad \text{chips}=5, \ \beta=50.
\end{equation}
This scheme penalizes inefficiency and favors faster, rule-compliant gameplay.

\subsection{Cumulative Learning Framework}

All four agents share a common deep Q-network, following a centralized cumulative learning scheme~\cite{curriculum}. Experiences from all players are stored in a shared buffer and used to update the policy. This design improves sample efficiency by exposing the network to a broader range of transitions, while maintaining decentralized execution during gameplay.

\subsection{Agent Training Workflow}

The overall agent training process is summarized in Algorithm~\ref{alg:multiagent}. At each episode, the environment is initialized and agents act according to the current policy. Valid actions are sampled based on the game phase. Transitions are stored in the shared buffer, and gradient updates are periodically applied to the network. Exploration decays over time, and the target network is periodically updated.

\begin{algorithm}
\caption{Multi-Agent Training for SLS}
\label{alg:multiagent}
\begin{algorithmic}[1]
\State Initialize environment \texttt{env} and agents with shared Q-network
\For{each episode $e = 1$ to $N$}
    \State Reset environment: $s_0 \gets \texttt{env.reset()}$
    \For{each step $t = 1$ to $T$}
        \State Identify current player $a \gets \texttt{env.current\_player()}$
        \State Determine game phase $\text{phase} \gets \texttt{env.get\_phase()}$
        \State Select action $a_t \in \mathcal{A}$ via $\epsilon$-greedy policy
        \State Execute $a_t$, observe $(s_{t+1}, r_t, \text{done})$
        \State Store $(s_t,a_t,r_t,s_{t+1})$ in shared buffer
        \If{buffer size $>$ batch size and $t \bmod 10 = 0$}
            \State Sample minibatch and update network
        \EndIf
        \If{\text{done}} \State \textbf{break} \EndIf
        \State $s_t \gets s_{t+1}$
    \EndFor
    \State Decay exploration rate; periodically update target network
\EndFor
\end{algorithmic}
\end{algorithm}





\iffalse

\section{Proposed Methodology}
\label{3sec:method}
\subsection{Preliminaries of Reinforcement Learning}
\label{sec:preliminaries}

Reinforcement Learning (RL) is a machine learning paradigm in which an agent learns to make decisions by interacting with an environment to maximize a cumulative reward. In RL, the problem is modeled as a Markov Decision Process (MDP), which consists of the following elements:

\begin{itemize}
    \item \textbf{State Space ($\mathcal{S}$):} The set of all possible states in which the agent can find itself. Each state $s \in \mathcal{S}$ provides relevant information about the environment at a given time step.
    
    \item \textbf{Action Space ($\mathcal{A}$):} The set of all possible actions the agent can take. An action $a \in \mathcal{A}$ selected by the agent at time step $t$ influences the next state of the environment.
    
    \item \textbf{Transition Function ($P$):} This function, $P(s'|s, a)$, defines the probability of transitioning from state $s$ to state $s'$ when the agent takes action $a$. In deterministic environments, this transition is often represented by a fixed mapping from $s$ and $a$ to $s'$.
    
    \item \textbf{Reward Function ($R$):} The reward function $R(s, a, s')$ provides a scalar reward signal to the agent based on the action taken at a particular state. The goal of the agent is to maximize the total accumulated reward over time.

    \item \textbf{Policy ($\pi$):} A policy $\pi(a|s)$ is a strategy that the agent uses to decide the action $a$ given a state $s$. The policy can be deterministic, where a specific action is chosen for each state, or stochastic, where actions are selected with certain probabilities.
\end{itemize}

The objective in RL is to find an optimal policy $\pi^*$ that maximizes the expected cumulative reward, often expressed as the return $G_t$, which is the sum of discounted future rewards:
\begin{equation}
    G_t = \sum_{k=0}^{\infty} \gamma^k R_{t+k+1},
\end{equation}
where $\gamma \in [0,1)$ is the discount factor that balances the importance of immediate and future rewards. 

To learn an optimal policy, various RL algorithms are applied, including value-based methods like Q-learning and Deep Q-Networks (DQN), policy-based methods, and actor-critic methods. The agent's learning process involves exploring different actions to understand their long-term benefits while also exploiting known information to maximize rewards based on prior knowledge.

\subsection{State, Action, and Reward Definition}

We define the game environment mathematically with the state, action, and reward as follows:

\paragraph{State ($\mathbf{s_t}$)}
The state $\mathbf{s_t}$ at time step $t$ captures all relevant information about the current game environment. It is structured as a vector with specific components representing the game board, player chips, eliminated chips, the current player, game phase, and step count:
\begin{equation}
\begin{split}
\mathbf{s_t} = \{ \text{Board State}, \text{Player Chips}, \text{Dead Chips}, \\
\text{Current Player}, \text{Game State}, \text{Steps} \}    
\end{split}
\end{equation}

The overall observation space size, denoted as $\text{total\_obs\_size}$, is computed as follows:
\begin{equation}
\begin{split}
\text{total\_obs\_size} = \text{num\_rows} \times \text{num\_players} \times \text{max\_pile\_size} + 
\\
\text{num\_players}^2 + 2 \times \text{num\_players} + 4 + 1
\end{split}
\end{equation}

Each term in this equation corresponds to a specific component of the state:

\begin{itemize}
    \item \textbf{Board State:} $\text{num\_rows} \times \text{num\_players} \times \text{max\_pile\_size}$. This term represents the current state of the game board. 
    \begin{itemize}
        \item \texttt{num\_rows} is the number of playable rows in the game.
        \item \texttt{num\_players} represents the number of players, each of whom has their own set of chips that can be placed in any row.
        \item \texttt{max\_pile\_size} is defined as $\text{num\_players} \times \text{max\_chips}$, where $\text{max\_chips}$ is the maximum number of chips a player can hold. This value represents the upper limit on the size of a pile, assuming every player has placed the maximum number of chips in a single row.
    \end{itemize}
    Therefore, $\text{num\_rows} \times \text{num\_players} \times \text{max\_pile\_size}$ captures all possible states of the board, accounting for each row, player, and pile configuration.

    \item \textbf{Player Chips:} $\text{num\_players}^2$. This term keeps track of the chips each player currently holds.
    \begin{itemize}
        \item Since each player can potentially hold chips that originated from any of the other players, we need a matrix-like structure with $\text{num\_players} \times \text{num\_players}$ entries to represent the state of chips per player.
        \item Each entry $(i, j)$ in this structure denotes the number of chips player $i$ holds from player $j$.
    \end{itemize}
    
    \item \textbf{Dead Chips:} $\text{num\_players}$. This term represents the chips belonging to players who have been eliminated.
    \begin{itemize}
        \item As each player can potentially be eliminated during the game, the status of each player's chips must be tracked, and a single entry for each player is sufficient to mark their chips as dead.
    \end{itemize}
    
    \item \textbf{Current Player:} $\text{num\_players}$. This term indicates which player is currently active.
    \begin{itemize}
        \item We use a one-hot encoded vector of length $\text{num\_players}$ to identify the current player at each step. A value of $1$ at the $i$-th position signifies that player $i$ is currently active.
    \end{itemize}
    
    \item \textbf{Game State:} A vector of length $4$, representing the current phase or state of the game. There are four possible game states:
    \begin{itemize}
        \item \texttt{choose\_pile}: The phase where the agent selects a pile from which to play.
        \item \texttt{choose\_chip}: The phase where the agent selects a chip to use in the chosen pile.
        \item \texttt{choose\_next\_player}: The phase where the agent selects the next player in the sequence.
        \item \texttt{eliminate\_chip}: The phase where the agent eliminates a chip, marking it as no longer in play.
    \end{itemize}
    Each of these states is represented by a unique one-hot encoding within the 4-element vector, indicating the current phase of the game.

    \item \textbf{Steps:} A scalar value indicating the number of steps taken in the current episode.
    \begin{itemize}
        \item This component provides a running count of the steps, which can help track the agent’s efficiency in gameplay. It may also be used in reward calculation to incentivize faster completion of tasks.
    \end{itemize}
\end{itemize}

\paragraph{Action ($a_t$)}
The action $a_t$ taken by an agent at time step $t$ is chosen from the action space $\mathcal{A}$, defined as:

\begin{equation}
    \mathcal{A} = \{0, 1, 2, 3, 4, 5, 6, 7, 8, 9\}
\end{equation}

The action space includes $10$ discrete actions, categorized as follows:
\begin{itemize}
    \item Actions $\{0, 1, 2, 3, 4, 5\}$ correspond to the selection of rows and are valid only in the \texttt{choose\_pile} state. Each action in this range selects one of the six rows available.
    \item Actions $\{6, 7, 8, 9\}$ correspond to the selection of players and are valid in the \texttt{choose\_chip}, \texttt{choose\_next\_player}, and \texttt{eliminate\_chip} states. Each of these four actions corresponds to a specific player, allowing for targeted choices during these phases.
\end{itemize}


\paragraph{Reward ($r_t$)}
The reward function $r_t$ is designed to encourage agents to make beneficial moves while penalizing illegal actions. Specifically:
\begin{itemize}
    \item A reward of $-5$ is given for every illegal move, discouraging agents from violating game rules.
    \item For each positive (legal) move, the agent receives an initial reward of $5$. However, this reward is dynamically adjusted to account for the number of chips and steps taken by the agent.
\end{itemize}

Since the number of chips is set to a constant of $5$ in our experiments, the reward adjustment is primarily influenced by the steps taken. The adjusted reward function is defined as:
 
\begin{equation}
    r_t = \min\left(5, \frac{5}{\alpha \cdot \text{steps}}\right)
\end{equation}

where the adjustment parameter $\alpha$ is given by:

\begin{equation}
    \alpha = \frac{15}{\text{chips} \times \beta}
\end{equation}

In this setup:
\begin{itemize}
    \item $\text{chips} = 5$, which is constant in our experiments.
    \item $\beta = 50$, a fixed scaling parameter to regulate the rate of reward decay.
\end{itemize}

The purpose of this dynamic reward adjustment is to incentivize the agents to complete their tasks with fewer steps. As the number of steps increases, the adjusted reward decreases, encouraging efficiency in gameplay and discouraging unnecessary actions.


\subsection{Cumulative Learning Framework}
We employ a cumulative learning \cite{curriculum} approach, where all four agents share a common learning network, such as a DQN. The centralized learning scheme allows the agents to:
\begin{itemize}
    \item Share experiences through a collective experience buffer.
    \item Update the shared policy network, benefiting from more diverse and comprehensive data.
\end{itemize}

\subsection{Pseudocode for Agent-Based Gameplay}

The pseudocode is presented in Algorithm 1.

\begin{algorithm}
\caption{Gameplay with Multiple Agents}
\begin{algorithmic}[1]
\State Initialize environment \texttt{env} and agents \texttt{agents} with a shared network
\For{each episode $e = 1$ to \texttt{num\_episodes}}
    \State Reset environment: $\mathbf{s_0} \gets$ \texttt{env.reset()}
    \State Initialize total rewards for all agents
    \For{each step $t = 1$ to \texttt{max\_steps}}
        \State Determine the current state type: $\text{state\_type} \gets \texttt{env.get\_state\_type()}$
        \State Select current agent $a \gets$ \texttt{env.current\_player\_index}
        \If{\texttt{state\_type} == \texttt{choose\_pile}}
            \State Choose action $a_t \in \{0, 1, 2, 3, 4, 5\}$ using policy: $a_t \gets \text{current\_agent.act}(\mathbf{s_t})$
        \Else
            \State Choose action $a_t \in \{6, 7, 8, 9\}$ using policy: $a_t \gets \text{current\_agent.act}(\mathbf{s_t})$
        \EndIf
        \State Execute action $a_t$, observe next state $\mathbf{s_{t+1}}$, reward $r_t$, and done flag
        \State Store experience $(\mathbf{s_t}, a_t, r_t, \mathbf{s_{t+1}}, \text{done})$ in shared memory
        \If{length of shared memory $>$ \texttt{batch\_size} and $t \mod 10 = 0$}
            \State Sample minibatch from shared memory
            \State Perform gradient descent on shared agent's network
        \EndIf
        \State Update total rewards for all agents
        \If{done}
            \State Break loop
        \EndIf
        \State Update state: $\mathbf{s_t} \gets \mathbf{s_{t+1}}$
    \EndFor
    \State Decay exploration rate of shared agent
    \If{$e \mod 500 = 0$}
        \State Save model weights and update target network
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}


\newpage

\\~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\~

\newpage 

\begin{algorithm}
\caption{Multi-Agent Training for SLS}
\label{alg:multiagent}
\begin{algorithmic}[1]
\State Initialize environment \texttt{env} and agents with shared Q-network
\For{each episode $e = 1$ to $N$}
    \State Reset environment: $s_0 \gets \texttt{env.reset()}$
    \For{each step $t = 1$ to $T$}
        \State Identify current player $a \gets \texttt{env.current\_player()}$
        \State Determine game phase $\text{phase} \gets \texttt{env.get\_phase()}$
        \State Select action $a_t \in \mathcal{A}$ via $\epsilon$-greedy policy
        \State Execute $a_t$, observe $(s_{t+1}, r_t, \text{done})$
        \State Store $(s_t,a_t,r_t,s_{t+1})$ in shared buffer
        \If{buffer size $>$ batch size and $t \bmod 10 = 0$}
            \State Sample minibatch and update network
        \EndIf
        \If{\text{done}} \State \textbf{break} \EndIf
        \State $s_t \gets s_{t+1}$
    \EndFor
    \State Decay exploration rate; periodically update target network
\EndFor
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{Gameplay with Multiple Agents}
\begin{algorithmic}[1]
\State Initialize environment \texttt{env} and agents \texttt{agents} with a shared network
\For{each episode $e = 1$ to \texttt{num\_episodes}}
    \State Reset environment: $\mathbf{s_0} \gets$ \texttt{env.reset()}
    \State Initialize total rewards for all agents
    \For{each step $t = 1$ to \texttt{max\_steps}}
        \State Determine the current state type: $\text{state\_type} \gets \texttt{env.get\_state\_type()}$
        \State Select current agent $a \gets$ \texttt{env.current\_player\_index}
        \If{\texttt{state\_type} == \texttt{choose\_pile}}
            \State Choose action $a_t \in \{0, 1, 2, 3, 4, 5\}$ using policy: $a_t \gets \text{current\_agent.act}(\mathbf{s_t})$
        \Else
            \State Choose action $a_t \in \{6, 7, 8, 9\}$ using policy: $a_t \gets \text{current\_agent.act}(\mathbf{s_t})$
        \EndIf
        \State Execute action $a_t$, observe next state $\mathbf{s_{t+1}}$, reward $r_t$, and done flag
        \State Store experience $(\mathbf{s_t}, a_t, r_t, \mathbf{s_{t+1}}, \text{done})$ in shared memory
        \If{length of shared memory $>$ \texttt{batch\_size} and $t \mod 10 = 0$}
            \State Sample minibatch from shared memory
            \State Perform gradient descent on shared agent's network
        \EndIf
        \State Update total rewards for all agents
        \If{done}
            \State Break loop
        \EndIf
        \State Update state: $\mathbf{s_t} \gets \mathbf{s_{t+1}}$
    \EndFor
    \State Decay exploration rate of shared agent
    \If{$e \mod 500 = 0$}
        \State Save model weights and update target network
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}




\begin{algorithm}[t]
\caption{Multi-Agent Training for SLS (shared value network)}
\label{alg:multiagent}
\begin{algorithmic}[1]
\Require Environment $\texttt{env}$; shared Q-network $Q_\theta$; target network $Q_{\bar\theta}$; replay buffer $\mathcal{B}$; batch size $m$; discount $\gamma$; update period $U$; target update period $C$; initial $\epsilon$ with decay to $\epsilon_{\min}$
\State Initialize $\theta$, copy to $\bar\theta$; clear $\mathcal{B}$
\For{episode $e = 1$ to $N$}
    \State $s_0 \gets \texttt{env.reset()}$
    \For{$t = 0$ to $T{-}1$}
        \State $p_t \gets \texttt{env.current\_player()}$ \Comment{current player index}
        \State $\phi_t \gets \texttt{env.get\_phase()}$ \Comment{game phase}
        \State $\mathcal{A}_t \gets \textsc{LegalActions}(s_t, \phi_t)$ \Comment{action mask}
        \State \textbf{with} prob. $\epsilon$: sample $a_t \sim \text{Unif}(\mathcal{A}_t)$
        \State \textbf{else}: $a_t \gets \arg\max_{a \in \mathcal{A}_t} Q_\theta(s_t,a)$
        \State $(s_{t+1}, r_t, \textit{done}) \gets \texttt{env.step}(a_t)$
        \State $\mathcal{B}.\textsc{Push}(s_t, a_t, r_t, s_{t+1}, \textit{done})$
        \If{$|\mathcal{B}| \ge m$ \textbf{and} $(t \bmod U = 0)$}
            \State $\{(s^i,a^i,r^i,{s'}^{i},d^i)\}_{i=1}^{m} \gets \mathcal{B}.\textsc{Sample}(m)$
            \State $y^i \gets r^i + \gamma(1-d^i)\max_{a' \in \mathcal{A}({s'}^{i})} Q_{\bar\theta}({s'}^{i},a')$
            \State $\theta \gets \theta - \eta \nabla_\theta \frac{1}{m}\sum_{i=1}^{m}\big(Q_\theta(s^i,a^i)-y^i\big)^2$
        \EndIf
        \If{$(t \bmod C = 0)$}
            \State $Q_{\bar\theta} \gets Q_\theta$ \Comment{hard target update; or use Polyak averaging}
        \EndIf
        \State $s_t \gets s_{t+1}$
        \If{\textit{done}} \textbf{break} \EndIf
        \State $\epsilon \gets \max(\epsilon_{\min},\, \lambda \epsilon)$ \Comment{decay per step or per episode}
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


\fi

==> 4_result.tex <==
\section{Experiments and Discussion}
\label{4sec:result}



\begin{figure*}[t]
    \centering
\scriptsize 
(a) \includegraphics[width=0.22\linewidth]{fig/DQN.png}
(b) \includegraphics[width=0.22\linewidth]{fig/DDQN.png}
(c) \includegraphics[width=0.22\linewidth]{fig/DuelingDQN.png}
(d) \includegraphics[width=0.22\linewidth]{fig/Random.png}
% \caption{Performance comparison of different agents. Each subfigure depicts reward trends across episodes.}
\caption{Performance comparison of different agents:
(a) DQN: reward vs. episodes,
(b) DQN: steps vs. episodes,
(c) DDQN: reward vs. episodes,
(d) DDQN: steps vs. episodes,
(e) Dueling DQN: reward vs. episodes,
(f) Dueling DQN: steps vs. episodes.}

    \label{fig:agent_performance}
\end{figure*}




\begin{table}[]
    \centering
    \caption{Agent Performance Metrics}
\begin{adjustbox}{width=\linewidth}
    \begin{tabular}{@{}lcccccccc@{}}
        \toprule
        \textbf{Agent} & \multicolumn{4}{c}{\textbf{Reward}} & \multicolumn{4}{c}{\textbf{Steps}} \\
        \cmidrule(r){2-5} \cmidrule(l){6-9}
        & \textbf{Mean} & \textbf{Stdev} & \textbf{Min} & \textbf{Max} & \textbf{Mean} & \textbf{Stdev} & \textbf{Min} & \textbf{Max} \\
        \midrule
        DQN & 103.40 & 42.31 & -313.45 & 189.24 & 61.16 & 14.51 & 27.00 & 162.00 \\
        DDQN & 108.44 & 44.95 & -279.13 & 191.38 & 61.23 & 14.18 & 28.00 & 165.00 \\
        Dueling DQN & 102.06 & 49.62 & -319.76 & 192.09 & 65.92 & 15.94 & 28.00 & 173.00 \\
        Random & -8.78 & 43.52 & -419.26 & 94.19 & 65.24 & 17.76 & 29.00 & 174.00 \\
        \bottomrule
    \end{tabular}
\end{adjustbox}
    \label{tab:agent_performance}
\end{table}



\subsection{Training and Hyperparameters}
In our experiments, we utilized three foundational deep reinforcement learning (DRL) algorithms—DQN, DDQN, and Dueling DQN—alongside a baseline random agent. Table~\ref{tab:agent_performance} summarizes the performance of each agent. The agents were implemented using TensorFlow, employing a simple feed-forward neural network architecture to approximate the Q-values. The primary hyperparameters used for training each agent are as follows:

\begin{itemize}
    \item \textbf{Discount Factor} ($\gamma$): 0.95
    \item \textbf{Initial Exploration Rate} ($\epsilon$): 1.0
    \item \textbf{Exploration Decay Rate} ($\epsilon_{\text{decay}}$): 0.995
    \item \textbf{Minimum Exploration Rate} ($\epsilon_{\text{min}}$): 0.01
    \item \textbf{Learning Rate}: 0.001
    \item \textbf{Batch Size}: 64
\end{itemize}

\subsection{Base Model Architecture}
Each agent's neural network follows a simple structure, described as follows:
\begin{itemize}
    \item \textbf{Input Layer:} Accepts the state vector of size $\text{state\_size}$
    \item \textbf{Hidden Layers:} Two fully connected layers, each with 64 neurons and ReLU activations
    \item \textbf{Output Layer:} A fully connected layer with linear activation, producing $\text{action\_size}$ outputs representing the Q-values for each action
\end{itemize}

The model is compiled with Mean Squared Error (MSE) loss and the Adam optimizer with a learning rate of 0.001.

\subsection{Reward Structure and Performance Analysis}

The maximum attainable reward in a game of \textit{So Long Sucker} (SLS) is approximately 200, which aligns with the reward function graph for our trained agents. This suggests that classical DRL algorithms like DQN, DDQN, and Dueling DQN effectively learn the rules and structure of SLS, despite its strategic complexity.

The persistent gap between human and agent performance stems from the game’s reliance on implicit reasoning and long-horizon credit assignment. For example, selecting the next player is a context-dependent move that can only be evaluated many steps later, posing difficulties for value-based learners. Moreover, occasional illegal actions reflect the challenge of encoding complex rules within tabular action spaces. These findings suggest that while classical DRL captures basic legality, advanced approaches such as hierarchical RL, rule-augmented critics, or negotiation-conditioned policies may be necessary for richer strategic play. 



% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{fig/DQN.png}
%         \caption{Performance metrics for DQN}
%         \label{fig:DQN}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{fig/DDQN.png}
%         \caption{Performance metrics for DDQN}
%         \label{fig:DDQN}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{fig/DuelingDQN.png}
%         \caption{Performance metrics for Dueling DQN}
%         \label{fig:DuelingDQN}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{fig/Random.png}
%         \caption{Performance metrics for Random Agent}
%         \label{fig:Random}
%     \end{subfigure}
%     \caption{Performance comparison of different agents. Each subfigure depicts reward trends across episodes.}
%     \label{fig:agent_performance}
% \end{figure}



